se(3)-TrackNet: Data-driven 6D Pose Tracking by Calibrating Image Residuals in Synthetic Domains

Tracking the 6D pose of objects in video sequences is important for robot manipulation. This task, however, introduces multiple challenges: (i) robot manipulation involves significant occlusions; (ii) data and annotations are troublesome and difficult to collect for 6D poses, which complicates machine learning solutions, and (iii) incremental error drift often accumulates in long term tracking to necessitate re-initialization of the object's pose. This work proposes a data-driven optimization approach for long-term, 6D pose tracking. It aims to identify the optimal relative pose given the current RGB-D observation and a synthetic image conditioned on the previous best estimate and the object's model. The key contribution in this context is a novel neural network architecture, which appropriately disentangles the feature encoding to help reduce domain shift, and an effective 3D orientation representation via Lie Algebra. Consequently, even when the network is trained only with synthetic data can work effectively over real images. Comprehensive experiments over benchmarks - existing ones as well as a new dataset with significant occlusions related to object manipulation - show that the proposed approach achieves consistently robust estimates and outperforms alternatives, even though they have been trained with real images. The approach is also the most computationally efficient among the alternatives and achieves a tracking frequency of 90.9Hz.

==> alg/sampling.tex <==
$T_{t-1}$: previous frame estimated pose \\
$N$: number of particles to sample \\
$I_{t}$: currently observed RGBD image \\
$M$: object CAD model \\
$P_{scene}$: currently observed point cloud (converted from RGBD image) \\

\begin{algorithm}[h]
\label{alg_base_sample}

\caption{{\sc SAMPLE\_INFERENCE\ ($T_{t-1}$,$N$,$I_{t}$,$M$,$P_{scene}$)} }
$LCP_{best} \gets 0$ \;
$T_{t} \gets I_{4\times 4} $\;
\For{$i\gets0$ \KwTo  $N$ }
{
    sample pose $T_{t-1}^{i}$ by adding purturbation to $T_{t-1}$ \;
    render image $I^{i}$ using pose $T_{t-1}^{i}$ \;
    \tcc{neural net predict relative transform}
    $\bigtriangleup T$ \gets $f(I^{i},I_{t})$ \; 
    $T_t^{i} \gets \bigtriangleup T \cdot T_{t-1}$ \;
    $M^i \gets transformation(M,T_t^{i}$) \;
    $LCP^{i} \gets evaluate\_pose\_score(M^i,P_{scene}$) \;

  \If {$LCP^{i} > LCP_{best}$}{
    $LCP_{best} \gets LCP^{i}$ \;
    $T_{t} \gets T_t^{i}$ \;
  }
}

\end{algorithm}


==> sections/previous_related_work.tex <==
\subsection{Data-driven 6D Pose Estimation}
Learning-based techniques have shown promise in directly regressing the 6D object pose \cite{xiang2017posecnn, wang2019densefusion} from raw image data. Nevertheless, given the  complexity of $SO(3)$ space large amount of pose annotated training data is required to achieve satisfactory results in practice. This is often more challenging than labeling for object classification or detection. Some data-driven techniques combine deep learning with traditional techniques like PnP \cite{tekin2018real, tremblay2018deep}. Although more data-efficient, this could be problematic in case of severe occlusions, and often require precisely calibrated camera intrinsic parameters for the PnP step. Given that pose is re-estimated in every frame, estimation techniques often trade-off speed for accuracy \cite{xiang2017posecnn,mitash2017improving}. This might not be desirable for the accompanying control pipeline. In contrast, the current work exploits temporal information and achieves better performance than the state-of-art single image pose estimation methods in a limited running time while using only synthetic data for training.

\subsection{6D Pose Tracking}
Pose tracking approach optimize for both the pose quality and the computation speed. Within the setup of the current work, where CAD models of object to be tracked is available beforehand, the approaches can be categorized as probabilistic-based or optimization-based. 

\noindent \textbf{Probabilistic-Based:} 
\cite{choi2013rgb} implemented an efficient particle filtering framework by harnessing the computation power of GPU, where likelihood is computed based on color, distance and normals. Nevertheless, the hand-designed likelihood functions fail to generalize to different lighting conditions or scenes with more challenging clutter. \cite{ren2017real} formulates the 6D pose tracking as a  maximum a posteriori estimation problem, where object shape is implicitly represented by 3D signed distance function. \cite{Wthrich2013ProbabilisticOT} explicitly models occlusions and shows great success in terms of robustness, whereas the pose accuracy is not precise enough for certain manipulation tasks. To ameliorate this problem, \cite{issac2016depth} applied Gaussian Filtering and achieves promising pose accuracy but introduces more frequent tracking loss in the process. Recent work, \cite{deng2019poserbpf} proposed a novel Rao-Blackwellized particle filtering framework that decouples the translation and rotation uncertainty, achieving the state-of-art 6D pose tracking performance on the YCB Video benchmark. However, in cases of severe occlusions, re-initialization from a reliable single image pose estimation method is required. 

\noindent \textbf{Optimization-Based:}
A number of methods proposed objective functions that capture the discrepancy between the current observation and previous state, and compute relative transformation based on the minima of their residual function \cite{schmidt2014dart,pauwels2015simtrack,pauwels2014real,schmidt2015depth,hebert2012combined,joseph2015versatile,zhong2019robust,tjaden2018region}. In particular, \cite{pauwels2015simtrack,schmidt2014dart} combines the energy of optical flow, AR flow and point-to-plane distance and solves it in the least-squares sense. However, the SIFT feature and optical flow limits its performance in pure rotation scenarios and often extensive hyper-parameter tuning is be required in order to adapt to new scenarios such as varying lighting conditions. \cite{schmidt2014dart} introduces a general framework for tracking articulated objects composed of rigid bodies connected through a kinematic tree. It extends the signed distance function representation to articulated objects and takes full advantage of highly parallel GPU algorithms for data association and pose optimization. Although promising results have been demonstrated, it can only handle articulated object pose tracking. \cite{tjaden2018region} derives a region-based cost function using temporally consistent local color histograms, which is then minimized in the Gauss-Newton optimization scheme. It has shown great success in application to augmented reality using a monocular camera. Nevertheless, when applied to robotics, it is not clear how it compares with other RGB-D based approaches when depth data is also available. Rooted from the idea of optical-flow estimation, more recent work \cite{li2018deepim} leverages the FlowNetSimple network \cite{fischer2015flownet} that is able to refine pose output from any 6D object pose detection approach, but also has an extension to RGB-based tracking. However, it requires frequent re-initialization and has to be trained on real and synthetic data.

\subsection{Simulation to Reality}
Training on synthetically generated datasets allow faster, more scalable, and lower-cost data collection \cite{tobin2017domain}. However, the discrepancy in appearance between the synthetic data and real ones often results in a significant performance drop when naively applying the models trained on synthetic images to real world. Domain adaptation techniques like Gradient-reversal \cite{ganin2014unsupervised} and utilizing Generative Adversarial Networks (GANs) for input space domain alignment \cite{shrivastava2017learning} help bridge this gap. These methods, however, often assumes the source domain already resembles the target domain to certain extent, which could not be trivially satisfied in practice.

Advancements in computer graphics, \cite{yosinski2014transferable} \cite{movshovitz2016useful,richter2016playing} have
shown the benefits of performing photo-realistic renderings on tasks such as object detection and viewpoint estimation when accounting for diverse object views and backgrounds. However, such photo-realistic image generation typically cannot be produced in current state-of-art robotics simulators \cite{xie2019best}, and often introduces another source of human involvement. \cite{tobin2017domain} explores domain randomization, a simple yet effective technique for synthetic data generation by randomizing rendering settings in the simulator. Transferability to real world has been demonstrated when the model is trained using only these domain randomized synthetic data. \cite{tremblay2018deep} inherits this idea but also combines it with photo-realistic rendering technique to perform competitively on YCB Video dataset \cite{xiang2017posecnn}. Our work, without using photo-realism, and just trained over synthetic training data can outperform state-of-art methods that are trained using partial real data over multiple benchmarks.

==> tables/compare_poserbpf.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|cccccccc|cc}
% \hline
%                          & \multicolumn{2}{c|}{PoseRBPF (50 particles)} & \multicolumn{2}{c}{PoseRBPF (200 particles)} & \multicolumn{2}{c}{PoseRBPF++ (200 particles)} & \multicolumn{2}{c|}{PoseRBPF (200 particles)} & \multicolumn{2}{c|}{Ours}        \\ \hline
% Modality                 & \multicolumn{2}{c|}{RGB}                     & \multicolumn{2}{c}{RGB}                      & \multicolumn{2}{c}{RGB}                        & \multicolumn{2}{c|}{RGBD}                     & \multicolumn{2}{c|}{RGBD}        \\ \hline
% Objects                  & ADD                  & ADD-S                 & ADD                  & ADD-S                 & ADD                   & ADD-S                  & ADD                   & ADD-S                 & ADD & \multicolumn{1}{c|}{ADD-S} \\ \cline{1-1} \cline{8-11} 
% 002\_master\_chef\_can   & 56.1                 & 75.6                  & 58.0                 & 77.1                  & 63.3                  & 87.5                   & 90.5                  & 95.1                  &     & \multicolumn{1}{c|}{}      \\
% 003\_cracker\_box        & 73.4                 & 85.2                  & 76.8                 & 87.0                  & 77.8                  & 87.6                   & 88.2                  & 93.0                  &     & \multicolumn{1}{c|}{}      \\
% 004\_sugar\_box          & 73.9                 & 86.5                  & 75.9                 & 87.6                  & 79.6                  & 89.4                   & 92.9                  & 95.5                  &     & \multicolumn{1}{c|}{}      \\
% 005\_tomato\_soup\_can   & 71.1                 & 82.0                  & 74.9                 & 84.5                  & 73.0                  & 83.6                   & 90.0                  & 93.8                  &     & \multicolumn{1}{c|}{}      \\
% 006\_mustard\_bottle     & 80.0                 & 90.1                  & 82.5                 & 91.0                  & 84.7                  & 92.0                   & 91.9                  & 96.3                  &     &                            \\
% 007\_tuna\_fish\_can     & 56.1                 & 73.8                  & 59.0                 & 79.0                  & 64.2                  & 82.7                   & 91.1                  & 95.3                  &     & \multicolumn{1}{c|}{}      \\
% 008\_pudding\_box        & 54.8                 & 69.2                  & 57.2                 & 72.1                  & 64.5                  & 77.2                   & 85.8                  & 92.0                  &     & \multicolumn{1}{c|}{}      \\
% 009\_gelatin\_box        & 83.1                 & 89.7                  & 88.8                 & 93.1                  & 83.0                  & 90.8                   & 96.3                  & 97.5                  &     & \multicolumn{1}{c|}{}      \\
% 010\_potted\_meat\_can   & 47.0                 & 61.3                  & 49.3                 & 62.0                  & 51.8                  & 66.9                   & 68.7                  & 77.9                  &     & \multicolumn{1}{c|}{}      \\
% 011\_banana              & 22.8                 & 64.1                  & 24.8                 & 61.5                  & 18.4                  & 66.9                   & 74.2                  & 86.9                  &     & \multicolumn{1}{c|}{}      \\
% 019\_pitcher\_base       & 74.0                 & 87.5                  & 75.3                 & 88.4                  & 63.7                  & 82.1                   & 86.8                  & 94.2                  &     & \multicolumn{1}{c|}{}      \\
% 021\_bleach\_cleanser    & 51.6                 & 66.7                  & 54.5                 & 69.3                  & 60.5                  & 74.2                   & 86.0                  & 93.0                  &     & \multicolumn{1}{c|}{}      \\
% 024\_bowl                & 26.4                 & 88.2                  & 36.1                 & 86.0                  & 28.4                  & 85.6                   & 25.5                  & 94.2                  &     & \multicolumn{1}{c|}{}      \\
% 025\_mug                 & 67.3                 & 83.7                  & 70.9                 & 85.4                  & 77.9                  & 89.0                   & 90.9                  & 97.1                  &     & \multicolumn{1}{c|}{}      \\
% 035\_power\_drill        & 64.4                 & 80.6                  & 70.9                 & 85.0                  & 71.8                  & 84.3                   & 93.9                  & 96.1                  &     & \multicolumn{1}{c|}{}      \\
% 036\_wood\_block         & 0                    & 0                     & 2.8                  & 33.3                  & 2.3                   & 31.4                   & 20.1                  & 89.1                  &     & \multicolumn{1}{c|}{}      \\
% 037\_scissors            & 20.6                 & 30.9                  & 21.7                 & 33.0                  & 38.7                  & 59.1                   & 76.1                  & 85.6                  &     & \multicolumn{1}{c|}{}      \\
% 040\_large\_marker       & 45.7                 & 54.1                  & 48.7                 & 59.3                  & 67.1                  & 76.4                   & 92.0                  & 97.1                  &     & \multicolumn{1}{c|}{}      \\
% 051\_large\_clamp        & 27.0                 & 73.2                  & 47.3                 & 76.9                  & 38.3                  & 59.3                   & 48.5                  & 94.8                  &     & \multicolumn{1}{c|}{}      \\
% 052\_extra\_large\_clamp & 50.4                 & 68.7                  & 26.5                 & 69.5                  & 32.3                  & 44.3                   & 40.3                  & 90.1                  &     & \multicolumn{1}{c|}{}      \\
% 061\_foam\_brick         & 75.8                 & 88.4                  & 78.2                 & 89.7                  & 84.1                  & 92.6                   & 81.1                  & 95.7                  &     & \multicolumn{1}{c|}{}      \\
% ALL                      & 57.1                 & 74.8                  & 59.9                 & 77.5                  & 62.1                  & 78.4                   & 80.8                  & 93.3                  &     & \multicolumn{1}{c|}{}      \\ \hline
% Speed (fps)              & \multicolumn{2}{c}{20.3}                     & \multicolumn{2}{c}{11.5}                     & \multicolumn{2}{c}{-}                          & \multicolumn{2}{c|}{5.0}                      & \multicolumn{2}{c|}{}            \\ \hline
% Re-initialization times  & \multicolumn{2}{c}{}                         & \multicolumn{2}{c}{}                         & \multicolumn{2}{c}{}                           & \multicolumn{2}{c|}{0}                        & \multicolumn{2}{c|}{0}           \\ \hline
% \end{tabular}%
% }
% \caption{}
% \label{tab:compare_poserbpf}
% \end{table*}

==> tables/dataset_summary.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
%                                                                           & YCB Video                                                                                             & Choi's                                                                   & T-LESS                                                                   & Issac's                                                                        & Lee's                                                                  & Krull's                                                                & Moving-YCB (ours)                                                                       \\ \hline
% camera used                                                                & RGBD                                                                                                  & RGBD                                                                     & RGBD                                                                     & Depth                                                                          & RGBD                                                                   & RGBD                                                                   & RGBD                                                                                    \\ \hline
% domain                                                                     & real                                                                                                  & synthetic                                                                & real                                                                     & real                                                                           & real                                                                   & real                                                                   & real                                                                                    \\ \hline
% scenario                                                                   & \begin{tabular}[c]{@{}c@{}}moving camera, \\ static objects\end{tabular}                              & \begin{tabular}[c]{@{}c@{}}moving camera, \\ static objects\end{tabular} & \begin{tabular}[c]{@{}c@{}}moving camera, \\ static objects\end{tabular} & \begin{tabular}[c]{@{}c@{}}moving object,\\ static camera\end{tabular}         & \begin{tabular}[c]{@{}c@{}}moving object,\\ static camera\end{tabular} & \begin{tabular}[c]{@{}c@{}}moving object,\\ static camera\end{tabular} & \begin{tabular}[c]{@{}c@{}}moving object,\\ static camera\end{tabular}                  \\ \hline
% object models                                                              & precisely scanned                                                                                     & reconstructed,not precise                                                & precisely scanned                                                        & no texture                                                                     & some have no texture                                                   & reconstructed,not precise                                              & precisely scanned                                                                       \\ \hline
% object categories                                                          & 21                                                                                                    & 4                                                                        & 30                                                                       & 6                                                                              & 8                                                                      & 4                                                                      &                                                                                         \\ \hline
% \begin{tabular}[c]{@{}c@{}}number of videos \\ for evaluation\end{tabular} & 12                                                                                                    & 4                                                                        & 20                                                                       & 37                                                                             & 8                                                                      & 8                                                                      &                                                                                         \\ \hline
% manipulator                                                                & -                                                                                                     & -                                                                        & -                                                                        & human hand                                                                     & human hand                                                             & human hand                                                             & \begin{tabular}[c]{@{}c@{}}vaccum gripper, Yale Hand T42, \\ Robotiq 2F-85\end{tabular} \\ \hline
% pose annotation                                                            & \begin{tabular}[c]{@{}c@{}}inferred from \\ camera trajectory \\ via global optimization\end{tabular} & from simulator                                                           & manually refined                                                         & \begin{tabular}[c]{@{}c@{}}acquired from motion \\ capture system\end{tabular} & manually refined                                                       & manually refined                                                       & manually refined                                                                        \\ \hline
% \end{tabular}%
% }
% % \caption{}
% \label{tab:dataset_compare}
% \end{table*}
